On the Structure of Polyhedral Products

In this thesis, we study the structure of the polyhedral product $\mathcal{Z}_{\mathcal{K}}(D^1,S^0)$ determined by an abstract simplicial complex ${\mathcal{K}}$ and the pair $(D^1,S^0)$. We showed that there is natural embedding of the hypercube graph in $\mathcal{Z}_{\mathcal{K}_n}(D^1,S^0)$ where ${\mathcal{K}}_n$ is the boundary of an $n$-gon. This also provides a new proof of a known theorem about genus of the hypercube graph. We give a description of the invertible natural transformations of the polyhedral product functor. Then, we study the action of the cyclic group $\mathbb{Z}_n$ on the space $\mathcal{Z}_{\mathcal{K}_n}(D^1,S^0)$. This action determines a $\mathbb{Z}[\mathbb{Z}_n]$-module structure of the homology group $H_*(\mathcal{Z}_{\mathcal{K}_n}(D^1,S^0))$. We also study the Leray-Serre spectral sequence associated to the homotopy orbit space $E\mathbb{Z}_n\times_{\mathbb{Z}_n} \mathcal{Z}_{\mathcal{K}_n}(D^1,S^0)$.

==> chapters/03-chapter.tex <==
\chapter{Chapter 3}
\label{chap:chapter-3}

\section*{}

% \subsection{This is a numbered second-level section head}
% This is an example of a numbered second-level heading.

% \subsection*{This is an unnumbered second-level section head}
% This is an example of an unnumbered second-level heading.

% \subsubsection{This is a numbered third-level section head}
% This is an example of a numbered third-level heading.

% \subsubsection*{This is an unnumbered third-level section head}
% This is an example of an unnumbered third-level heading.

Real moment angle complex or polyhedral products are special kind of subspaces of product spaces. The topological structure of $\Z_\K(D^1,S^0)$ can be very complicated depending on the simplicial complex $\K$. Li Cai has given a proof in \cite{C}(theorem 2.3) that $\Z_\K(D^1,S^0)$ is a homology $n$-manifold if and only if $\abs{\K}$ is a generalized homology $n$-sphere. In this paper we first give a proof of the known fact that if $\abs{\K}$ is a homeomorphic to $S^{n-1}$ then $\Z_\K(D^1,S^0)$ is a (closed) $n$-dimensional topological manifold. If we use Poincare conjecture, we can also imply that a necessary and sufficient condition for $\Z_\K(D^1,S^0)$ to be a (closed) manifold is that $\abs\K$ is a sphere. We give a proof by using the geometric construction of $\Z_\K(D^1,S^0)$ and embedding of $con(\abs{\K})$ in $[0,1]^m$. We also give an inductive prove of the fact that if $\abs\K$ is an $n$-gon, then $\Z_\K(D^1,S^0)$ will be an oriented surface of genus $1+(n-4) 2^{n-3}$ for $n\geq 3$.
\section{Moment Angle Complex}
\begin{definition}
Let $\K$ be an abstract simplicial complex on $m$ vertices with $[m] = \{1,\dots,m\} $ and let $(\underline{X}, \underline{A}):= \{(X_i, A_i)\}_{i\in [m]}$ be a collection of pairs of pointed spaces indexed by the vertex set of $K$. The polyhedral product $\mathcal{Z}_\K(\underline{X}, \underline{A})$ is defined by
$$
\mathcal Z_\K(\underline{X}, \underline{A}) := \bigcup_{\sigma \in K} (\underline{X}, \underline{A})^\sigma
$$
where 
$$ (\underline{X}, \underline{A})^\sigma = Y_1\times ...\times Y_m, \text{ where } 
Y_i = \begin{cases}
X_i \ \text{ if } i\in \sigma\\
A_i \ \text{ if } i\notin \sigma\\

\end{cases}
$$ 

\end{definition}
\begin{example}
Let $\K$ be the boundary of a triangle and $$(\underline{X}, \underline{A}) = {\{(D^1,S^0)\}}_{i\in \{0,1,2\}}$$ Denote the polyhedral product by $\mathcal{Z}_K(D^1,S^0)$. By the above definition, 

\begin{align*}
\mathcal{Z}_\K(D^1,S^0) &= (D^1\times D^1\times S^0) \cup (S^0 \times D^1\times D^1) \cup (D^1\times S^0\times D^1)\\
& = \partial(D^1\times D^1\times D^1)\\
& \approx \partial D^3 \approx S^2.
\end{align*}

\end{example}
So $\Z_\K(D^1,S^0)$ is a topological manifold when $\K$ is the boundary of a triangle. Depending on the shape of $\K$, the moment angle complex $\Z_\K(D^1,S^0)$ can be very complicated. 
\begin{example}
Let $\K$ be the graph in figure \ref{fig:my_label1}.   
\begin{figure}
    \centering
\begin{tikzpicture}
    \node[main node] (1) {$1$};
    \node[main node] (2) [below left = 1cm and .6cm of 1]  {$2$};
    \node[main node] (3) [below right = 1cm and .6cm of 1] {$3$};
    \node[main node] (4) [right = 1cm of 3] {$4$};

    \path[draw,thick]
    (1) edge node {} (2)
    (2) edge node {} (3)
    (3) edge node {} (1)
    (3) edge node {} (4);
    
\end{tikzpicture}

    \caption{A graph with 4 vertices}
    \label{fig:my_label1}
\end{figure}

Then
\begin{align*}
\mathcal{Z}_\K(D^1,S^0) &=  (\partial(D^1\times D^1\times D^1) \times S^0) \cup (S^0\times S^0 \times D^1 \times D^1)\\
\end{align*}
which is not a topological manifold. This space is homeomorphic to figure \ref{fig:my_label2} which is actually boundary of two copies of $3$-dimensional cube with four strips attached to it. 

\begin{figure}
    \centering
    \includegraphics[scale = 0.5]{figures/mom_angle_example.eps}
    \caption{$\Z_\K$ is not a topological manifold.}
    \label{fig:my_label2}
\end{figure}


\end{example}

We first prove that $\Z_\K(D^1,S^0)$ is a topological manifold if $\K$ is an $n$-gon. We will give an inductive proof and also show that it is an oriented surface. This space is regarded as 'regular topological skew polyhedra' in the 1938 work of Coxeter \cite{Cox}.
\begin{lemma}
Let $\K_n$ be the boundary of an $n$-gon($n\geq 3$). Then $\mathcal{Z}_{\K_n}(D^1,S^0)$ is a (closed) topological manifold of dimension 2. Moreover, it is oriented with genus $1+(n-4) 2^{n-3}$.
\begin{proof}
Denote $\mathcal{Z}_{\K_n}(D^1,S^0)$ by only $\mathcal{Z}_{\K_n}$.
We will prove by induction. For $n = 3$, it is straightforward by previous example. 
Let's assume the statement is true for $n = m $. So $\mathcal Z_{\K_m}$ is an oriented surface of genus $1+(m-4)2^{m-3}$. Also note that

\begin{align*}
\mathcal Z_{\K_m} = &\ \ \overbrace {D^1\times D^1\times S^0\times \cdots \cdots \cdots\times S^0}^{n factors} \\
      & \cup S^0\times D^1\times D^1\times S^0\times \cdots \times S^0 \\
      & \ \ \vdots\\
      & \cup S^0\times \cdots \cdots \cdots \times S^0\times   D^1\times D^1 \\
      & \cup D^1\times S^0 \cdots \cdots \cdots \cdots \times   S^0\times D^1 \\
\end{align*}
Let $X$ be the last term in the union that is $ X =  D^1\times S^0 \cdots \cdots \cdots \cdots \times   S^0\times D^1 \subset \mathcal{Z}_{\K_m}$. By induction hypothesis, $\mathcal{Z}_{\K_m}$ is an oriented surface of genus $1+(m-4)2^{m-3}$. And $X$ is $2^{m-2}$ copies of $D^1\times D^1$ on that surface. Now note that, $$\partial (X) = (S^0\times S^0 \cdots \cdots \cdots \cdots \times   S^0\times D^1) \cup (D^1\times S^0 \cdots \cdots \cdots \cdots \times   S^0\times S^0) $$ and
$$
\mathcal{Z}_{\K_{m+1}} = ((\mathcal{Z}_{\K_m}-X)\times S^0)\cup (\partial X\times D^1) 
$$
This means that to construct $\mathcal{Z}_{\K_{m+1}}$, we first delete $2^{m-2}$ copies of $D^1\times D^1$ from $\mathcal{Z}_{\K_m}$, then take two copies of $\mathcal{Z}_{\K_m}-X$ and glue $2^{m-2}$ copies of 1-handle along the boundary of $X$. So clearly $\mathcal{Z}_{\K_{m+1}}$ is an oriented surface. 

Now to calculate the genus, let $g_m$ denote the genus of $\mathcal{Z}_{\K_m}$. So by the avobe construction we have,
$$
g_3 = 0,\  g_{m+1} = 2g_m + 2^{m-2}-1
$$
which has solution
$$
g_m= 1 + (m-4)2^{m-3}
$$
\end{proof}

\end{lemma}

In a more general situation, if $\K$ is a triangulation of a sphere then $\Z_\K(D^1,S^0)$ is a topological manifold. A proof for $\Z_\K(D^2,S^1)$ can be found in \cite{BT}. We will prove the statement for real moment angle complex $\Z_\K(D^1,S^0)$.

\begin{theorem}
If $\K$ is a triangulation of an $(n-1)$-dimensional sphere, then $\mathcal{Z}_\K(D^1,S^0)$ is an $n$-dimensional (closed) topological manifold.
\end{theorem}

To prove this proposition we will need some construction and give a new definition of moment angle complex which is equivalent to definition $1.1$.
\begin{definition}
The \textit{barycentric subdivision} of an abstract simplicial complex $\K$ is the simplicial complex $\K'$ with vertex set $\{I\subset \K, \ I\neq \varnothing \}$ and  simplices $\{\{I_1,\cdots,I_r\}\subset \K : \varnothing \neq I_1 \subset \cdots \subset I_r\}$.
\end{definition}
\begin{construction}[{embedding of $\abs{con(\K')}$ in $\mathbb I ^m $}] 
\label{con}
Let $\K$ be a simplicial complex on $[m] = {1,\dots, m}$ and $\mathbb I^m = \{(y_1,\cdots,y_m): 0\leq y_i\leq 1\}$ denote the unit cube in $\mathbb R^m _{\geq0}$. All the faces of $\mathbb I^m$ have the form 
$$
C_{J\subset I} = \{(x_1,\cdots,x_m)\in \mathbb{I}^m : x_j = 0\ \forall j\in J \text{ and } x_i = 1\ \forall i\notin I \}
$$
where $J\subset I$ is a pair of subsets of $[m]$. Also denote $C_{\varnothing\subset I}$ by $C_{I}$. Now assign to a subset $I = \{i_1,\dots , i_k\} \subset [m]$ the vertex $v_I = C_{I\subset I}$ of $\mathbb{I}^m$. So, $v_I = (x_1,\cdots, x_m)$ where $x_i = 0$ if $i\in I$ and $x_i = 1$ otherwise. Considering each subset $I \subset [m]$ as a vertex of $\K'$, we can extend this mapping to a piecewise linear embedding $ i_c: \K' \to  \I^m$. Note that under this embedding, each vertex of $\K'$ is mapped to a vertex of $I^m$ where at least one coordinate is $0$. So $\K'$ is embedded in $\I^m \cap Bd(\R^m_{\geq0})$. Now we can map the cone vertex  to $(1,\cdots,1)\in \I^m$ and extend our map to a piecewise linear map $con(i_c): \abs{con(\K')} \to \I^m$. Denote the image of this embedding in $\I^m$ by $cc(K)$. This construction is explained in more detail in \cite{BT} p. 85. For example, figure \ref{fig:my_label3} shows $cc(\K)$ when $\K$ is the boundary of a triangle.

\begin{figure}
    \centering
    \includegraphics[scale = 0.8]{figures/cubical_cpx.eps}
    \caption{$\K$, a triangle and it's cubical complex $cc(\K)$.}
    \label{fig:my_label3}
\end{figure}



\end{construction}


\begin{definition}
The moment angle complex $\Z_\K(D^1,S^0)$ is defined as the pullback of the following diagram 
\begin{displaymath}
    \xymatrix{ \Z_\K(D^1,S^0) \ar[r] \ar[d] & [-1,1]^m  \ar[d]^\rho \\
                cc(\K) \ar@{^{(}->}[r] & \I^m  }
\end{displaymath}
where $\rho$ is defined as $\rho(u_1,\cdots,u_m) = (u_1^2,\cdots, u_m^2)$. Explicitly, we have $$\Z_\K(D^1,S^0) = \rho^{-1}(cc(\K))$$
\label{zk}
\end{definition}

One important observation: from the definition we note that $\Z_\K(D^1,S^0)$ is obtained by reflecting $cc(\K)\subset \I^m$ at all coordinate planes. Now we can prove proposition $1.5$.

\begin{proof}[(proof for theorem 1.5)] 
Let $\K$ be a triangulation of an $(n-1)$-dimensional sphere with $m$ vertices. Then $\abs{\K'}$ is also a $(n-1)$-dimensional sphere, and $\abs{con(\K')}$ is a topological manifold (it's an $n$-dimensional closed ball) with boundary $\abs{\K'} \approx S^{n-1}$. Under the above construction $1.7$, we can embed this cone on $\I^m$ with the boundary $\abs{\K'}$ embedded in the coordinate planes of $\R^m_{\geq 0}$. Since the cone vertex is mapped to $(1,\cdots, 1) \in \I^m$, we have $cc(\K)\cap \R^m_{\geq 0} = Bd(con(|\K'|))$ which is exactly the embedding of $\abs{\K'}$. Now if we reflect this embedding on each coordinate plane of $\R^m$ we will get a topological manifold of dimension $n$. Since we are reflecting along the boundary, this topological manifold is a closed manifold. This completes the proof of proposition $1.5$.
\end{proof}

Now consider the converse of the problem. If  $\K$ is a simplicial complex on $[m]$ and $\Z_\K(D^1,S^0)$ is an $n$-dimensional (closed) manifold, what can we tell about $\abs{K}$?
From the above definition and construction, it is clear that if $\mathcal Z_\K(D^1,S^0)$ is a topological manifold, then $cc(\K)$ must be an $n$-dimensional topological manifold (with boundary $\abs{\K'}$). But $cc(\K)$ is an embedding of $\abs{con(\K')}$ in the boundary of $\mathbb I^m$ (Construction \ref{con}). So we get, $\abs{con(\K')}$ is also a topological manifold with boundary $\abs{\K'}$. First we will prove that $\abs\K'$ must be simply connected and use this with the Poincare conjecture to show that it is a sphere. A related question has been discussed at \cite{MO}. 

\begin{proposition}\label{my_prop2}
If $X \subset \R^m$ and $CX \ (con(X))$ is a topological manifold with dimension $n\geq 2$ and boundary $X$, then $X$ is simply connected.
\begin{proof} 
First we will prove $X$ is path connected. Let the cone vertex of $CX$ be P. Take two points $A,B$ in $X$. Since $CX$ is a topological manifold, point $P$ has an open neighbourhood $U$ homeomorphic to $\R^n$. Since $n\geq 2$, $U-\{P\}$ must be path connected. Note that line segments $A\times [0,1]$ and $B\times [0,1]$ must intersect this open neighborhood $U$ at some points $A'$ and $B'$ other than the cone vertex $P$. So there exist a path $p'$ in $U-{P}$ connecting $A'$ and $B'$. Since $CX=\frac{X\times [0,1]}{X\times \{1\}}$, we can consider $U-\{P\}$ as a subspace of $X\times[0,1)$ and project the path $p'$ to a path $p$ in $X$. Clearly, $p(0)=A$ and $p(1)=B$. So $X$ is path connected.

To prove that $X$ is simply connected we will use Van Kampen theorem. Let $V = CX - \{P\}$ and $U\approx R^n$ be a neighborhood of $P$ (this is possible since $CX$ is a topological manifold). Note that $V$ is path connected since $X$ is path connected. Also, $U$ is path connected. For $n\geq 2$, we have $U\cap V = U - \{P\}$ is homeomorphic to $\R^n - \{pt\}$ which is simply connected. So by Van Kampen theorem, 
$$
\pi_1(CX) \cong \pi_1(V)* \pi_1(U)
$$
But $\pi_1(U)$ is trivial since $U\approx \R^n $ for $n\geq 2$ and $\pi_1(V) \cong \pi_1(X) $ since $X$ is homotopy equivalent to $CX-\{P\}$. Also, we know that cone of any space is contractible so $\pi_1(CX) = 0$. This implies that, $\pi_1(X) = 0$. 
\end{proof}
\label{my_prop1}
\end{proposition}

To prove our result, we also need the following well known theorems in algebraic topology. More detail can be found in \cite{H} chapter 4.

\begin{theorem}[Whitehead's Theorem]
If a map $f: X\to Y$ between connected CW complexes induces isomorphisms
$f_? : \pi_n(X)\to \pi_n(Y )$ for all n, then $f$ is a homotopy equivalence. In case $f$ is
the inclusion of a subcomplex $X\hookrightarrow Y$ , the conclusion is stronger: $X$ is a deformation
retract of $Y$.
\end{theorem}

\begin{theorem}[Hurewicz's Theorem]
If a space $X$ is $(n - 1)$-connected, $n \geq 2$, then $\tilde{H}_i(X) = 0$ for $i < n$
and $\pi_n(X) \cong H_n(X)$. If a pair $(X, A)$ is $(n - 1)$-connected, $n \geq 2$, with A simply connected and nonempty, then $H_i(X, A) = 0$ for $i < n$ and $\pi_n(X, A) \approx H_n(X, A)$.
\end{theorem}

Using the Hurewicz theorem, we can get a homology version of the Whitehead's theorem.
\begin{corollary}\label{my_cor1}
A map $f : X\to Y$ between simply-connected CW complexes is a homotopy
equivalence if $f_* : H_n(X)\to H_n(Y )$ is an isomorphism for each $n$. 
\begin{proof}
A proof can be found in \cite{H} corollary 4.33.
\end{proof}
\end{corollary}

\begin{proposition}\label{my_prop3}
If $X$ (CW complex) is simply connected homology sphere, then $X$ is a homotopy sphere.
\begin{proof}
It follows directly from corollary \ref{my_cor1}.
\end{proof}
\end{proposition}

\begin{proposition}\label{my_prop4}
If $X$ is a topological space which is realized by a simplicial complex $\K$ on $[m] $(therefore, $X = \abs\K$) and $CX$ is an $n$-dimensional topological manifold with boundary $X$ with $n\geq 3$, then $X$ must be a homology $(n-1)$-sphere.
\begin{proof}
By proposition \ref{my_prop1}, we know that $X$ is simply connected. Now we will show that $X$ is a homology sphere. Note that $X$ itself is a closed topological manifold since $X$ is the boundary of $CX$. Now consider $n\geq 2$ ($n=1$ to be showed). Let $P$ be the cone vertex, $U$ be a neighbourhood of $P$ homeomorphic to open ball $\mathring{D}^n$, $V$ be $CX-{P}$. So We have $U\cup V = CX, U\cap V \simeq S^{n-1}, V\simeq X$. Now we can use Mayer-Vietoris sequence,
$$
\begin{aligned}
\cdots \to H_n(U\cap V) \to H_n(U)\oplus H_n(V)\to H_n(CX)\to \cdots \\ \to H_0(U\cap V) \to H_0(U)\oplus H_0(V)\to H_0(CX)\to 0
\end{aligned}
$$
Since $CX$ and $U$ are contractible we have $H_n(CX) = H_n(U) = 0$. Also by the homotopy equivalence, we have $H_n(U\cap V) = H_n(S^{n-1}),\ H_n(V) = H_n(X)$. Combining all this information, we get 
$$
H_n(X) \cong H_n(S^{n-1})
$$
This completes the proof that $X$ is a homology $(n-1)$-sphere.
\end{proof}
\end{proposition}
We have all the ingredients to prove our main theorem. One final result we will need is the famous Poincare conjecture. The proof and discussion about the Poincare conjecuture is out of the scope of this paper. But we will use it as a blackbox to deduce our result. A detailed discussion can be found in \cite{SS,MF,GP1,GP3,GP2}.
\begin{theorem}[Generalized Poincare Conjecture]
A closed $n$-dimensional topological manifold which is homotopy equivalent to the $n$-sphere is homeomorphic to the standard $n$-sphere $S^n$.
\end{theorem}
Now we can prove our result. 
\begin{theorem}
Let $\K$ be a simplicial complex on $[m]$. If $\mathcal{Z}_\K(D^1,S^0)$ is a closed $n$-dimensional topological manifold, then $\K$ is a triangulation of the sphere $S^{n-1}$. 
\begin{proof}
%\fbox{ $n = 1$ case tbd}\\
\textbf{Case 1:}
($n=1$). By the definition of moment angle complex each maximal face of $\K$ is an $1$-element set. So $K$ is just bunch of points. By the construction \ref{con}, we can easily see that the cone vertex of $con(\K')$ must have a neighborhood homeomorphic to $\R$. Therefore, $\K$ must have two distinct vertices. So $\abs{\K}$ is homeomorphic to $S^0$.

\textbf{Case 2:}
($n=2$). All the maximal faces of $\K$ must have $2$-vertices. So $\K$ must be a graph. It is a connected graph, otherwise the cone vertex of $con(\K')$ cannot have a euclidean neighborhood. Also, each vertex must have two edges, otherwise $\Z_\K$ can not be a $2$-dimensional manifold. If some vertex has more than or equal to three edges, then $\Z_\K$ contains a subspace homeomorphic to $D^1\times (D^1\times S^0\times S^0\cup S^0\times D^1\times S^0\cup S^0\times S^0\times D^1)$, but this cannot be a subspace of a 2-dimensional manifold. So $\K$ is finite connected graph with each vertex having two edges, so $\K$ must be the boundary of an $n$-gon.

\textbf{Case 3:}
($n\geq 3$). By definition \ref{zk}, we know that $\Z_\K(D^1,S^0)$ can be obtained by reflecting $cc(\K)\subset \I^m$ to the $m$ coordinate hyperplanes in $\R^m$. So, if $\Z_\K$ is an closed $n$-manifold, then $cc(\K)\subset \I^m$ is an $n$-manifold with boundary embedded in the coordinate hyperplanes of $\R^m$. But topologically, $cc(\K)$ is homeomorphic to $con(\abs{\K'})$, where $\K'$ is the barycentric subdivision of $\K$. So the boundary of $cc(\K)$ is $\abs{\K'}$ which is embedded in the coordinate hyperplanes. Since $cc(\K) = con(\abs{\K'})$ is an $n$-manifold with boundary $\abs{\K'}$, by proposition \ref{my_prop2} , $\abs{\K'}$ is simply connected and by proposition \ref{my_prop4} , $\abs{\K'}$ is a homology $(n-1)$-sphere. Also by proposition \ref{my_prop3}, $\abs{\K'}$ must be a homotopy $(n-1)$-sphere. Now by the Poincare conjecture, we can say that $\abs{\K'}$ is homeomorphic to $S^{n-1}$. For any simplicial complex we have $\abs{K} \approx \abs{K'}$, so the conclusion follows.
\end{proof}
\end{theorem}

==> urcsmacros.tex <==
%
% urcsmacros
%
% author: Lawrence A. Crowl
% last updated: 28 April 1990
%
% BibTeX
%
\newcommand{\BibTeX}{{B\kern-.0833em{\sc ib}\kern-.1667em%
T\kern-.1667em\lower.5ex\hbox{E}\kern-.125emX}}
%
% SLiTeX
%
\newcommand{\SliTeX}{{\rm S\kern-.06em{\sc l\kern-.035emi}\kern-.06em
T\kern -.1667em\lower.7ex\hbox{E}\kern-.125emX}}
%
% UNIX
%
\newcommand{\UNIX}{{\sc Unix}}
%
% trademark
%
\newcommand{\trademark}{$^{\rm TM}$}
%
% singlespacing (for use in doublespaced documents)
%
\def\doublespacefactor#1#2{%
\newenvironment{singlespace}{\baselineskip #2\baselineskip}%
{\par \baselineskip #1\baselineskip}%
\par \baselineskip #1\baselineskip}
%
% various latin abbreviations
%
\def\adhoc{{\em ad hoc}}
\def\aposteriori{{\em a posteriori}}
\def\apriori{{\em a priori}}
\def\Cf{{\em Cf.}}
\def\cf{{\em cf.}}
\def\Eg{{\em E.g.}}
\def\eg{{\em e.g.}}
\def\etal{{\em et al.}}
\def\etc{{\em etc.}}
\def\Ibid{{\em Ibid.}}
\def\ibid{{\em ibid.}}
\def\Id{{\em Id.}}
\def\id{{\em id.}}
\def\Ie{{\em I.e.}}
\def\ie{{\em i.e.}}
\def\Loccit{{\em Loc.\ cit.}}
\def\loccit{{\em loc.\ cit.}}
\def\Opcit{{\em Op.\ cit.}}
\def\opcit{{\em op.\ cit.}}
\def\qv{{\em q.v.}}
\def\Qv{{\em Q.v.}}
\def\viz{{\em viz.}}
%
% andbreak  (for breaking author lists)
%
\def\andbreak{%% \begin{tabular}
\end{tabular}\\\begin{tabular}[t]{c}%% \end{tabular}
}
%
% titlequote
%
\def\titlequote#1{\hfill
\parbox{4in}{\begin{flushright}{\small\it #1}\end{flushright}}}
%
% weekdaystring
%
% Dump the day of the week in string form.
% This macro is only valid from 1901 A.D. through 2099 A.D.
%
\def\weekdaystring#1#2#3{{% extra brace saves enclosing register state
%
% days through the end of the year
% days := current year * 365
\count10=#3%
\multiply\count10 by 365%
% leap years := year / 4
\count11=#3%
\divide\count11 by 4%
% days := days + leap years
\advance\count10 by \count11
%
% find out if the current year is a leap year
% last leap year := leap years * 4
\count12=\count11%
\multiply\count12 by 4
% years since last leap year := current year - last leap year
\count13=#3%
\advance\count13 by -\count12%
% years since last leap year equals zero when current year is a leap year
%
% subtract off those days in this month and the following months
% days = days - following days [ is leap ] [ current month ]
\ifcase#2%
\or\ifcase\count13\advance\count10 by -366% leap January
\else\advance\count10 by -365% normal January
\fi%
\or\ifcase\count13\advance\count10 by -335% leap February
\else\advance\count10 by -334% normal February
\fi%
\or\advance\count10 by -306% March
\or\advance\count10 by -275% April
\or\advance\count10 by -245% May
\or\advance\count10 by -214% June
\or\advance\count10 by -184% July
\or\advance\count10 by -153% August
\or\advance\count10 by -122% September
\or\advance\count10 by -92% October
\or\advance\count10 by -61% November
\or\advance\count10 by -31% December
\fi%
%
% update days by day of month
% days := days + current day
\advance\count10 by #1%
%
% find weekday number
% offset for initial day of the week
\advance\count10 by 5
% last monday := (current day / 7) * 7
\count14=\count10%
\divide\count14 by 7%
\multiply\count14 by 7
% weekday number := current day - last monday
\count15=\count10%
\advance\count15 by -\count14
%
% now dump out appropriate string
\ifcase\count15 Monday\or Tuesday\or Wednesday%
\or Thursday\or Friday\or Saturday\or Sunday\fi%
}}
%
% monthstring
%
% Dump the month in string form.
%
\def\monthstring#1{\ifcase#1\or January\or February\or March\or April\or May%
\or June\or July\or August\or September\or October\or November\or December\fi}
%
% dateWDMY
%
% Redefine \today as "weekdaystring daynumber monthstring yearnumber" format.
%
\def\dateWDMY{\def\today{\weekdaystring{\day}{\month}{\year}\space%
\number\day\space\monthstring{\month}\space\number\year}}
%
% dateDMY
%
% Redefine \today as "daynumber monthstring yearnumber" format.
%
\def\dateDMY{\def\today{\number\day\space\monthstring{\month}%
\space\number\year}}
%
% dateWMDY
%
% Redefine \today as "weekdaystring monthstring daynumber, yearnumber" format.
%
\def\dateWMDY{\def\today{\weekdaystring{\day}{\month}{\year}\space%
\monthstring{\month}\space\number\day,\space\number\year}}
%
% dateMDY
%
% Redefine \today as "monthstring daynumber, yearnumber" format.
%
\def\dateMDY{\def\today{\monthstring{\month}\space\number\day,%
\space\number\year}}
%
% dateMY
%
% Redefine \today as "monthstring yearnumber" format.
%
\def\dateMY{\def\today{\monthstring{\month}\space\number\year}}
%
% dateY
%
% Redefine \today as "yearnumber" format.
%
\def\dateY{\def\today{\number\year}}
